Towards Practical Verification of Machine Learning: The Case of Computer Vision Systems

Due to the increasing usage of machine learning (ML) techniques in security- and safety-critical domains, such as autonomous systems and medical diagnosis, ensuring correct behavior of ML systems, especially for different corner cases, is of growing importance. In this paper, we propose a generic framework for evaluating security and robustness of ML systems using different real-world safety properties. We further design, implement and evaluate VeriVis, a scalable methodology that can verify a diverse set of safety properties for state-of-the-art computer vision systems with only blackbox access. VeriVis leverage different input space reduction techniques for efficient verification of different safety properties. VeriVis is able to find thousands of safety violations in fifteen state-of-the-art computer vision systems including ten Deep Neural Networks (DNNs) such as Inception-v3 and Nvidia's Dave self-driving system with thousands of neurons as well as five commercial third-party vision APIs including Google vision and Clarifai for twelve different safety properties. Furthermore, VeriVis can successfully verify local safety properties, on average, for around 31.7% of the test images. VeriVis finds up to 64.8x more violations than existing gradient-based methods that, unlike VeriVis, cannot ensure non-existence of any violations. Finally, we show that retraining using the safety violations detected by VeriVis can reduce the average number of violations up to 60.2%.

==> background.tex <==
\section{Background}

\subsection{Computer Vision Systems}
The main component of any computer vision system is an underlying machine learning (ML) component, which is capable to percept high-dimensional vision input that traditional software module cannot handle well. 
In general, ML model is a function $f: \mathbb{X}\rightarrow \mathbb{Y}$ mapping the input $\bm{x}\in \mathbb{X}$ (\eg images) to outputs $\bm{y}\in \mathbb{Y}$.
In image classification, $Y$ are discrete labels (\eg assign labels of cat or dog given an image), while in image regression, $Y$ is continuous value (\eg predicts steering angle given driving scenario captured from self-driving car's front camera).

In production, the vision system preprocesses inputs to conform to the input format of the ML model.
For example, a typical state-of-the-art ML model using deep learning (\eg Xception~\cite{chollet2016xception}) takes $299\times 299$ input image size (width$\times$height)

In this paper, we assume blackbox access to the ML model of computer vision systems, and thus we do not have any knowledge about the internal trained parameters.

\subsection{Image Transformation}
\label{subsec:image_transformation}
Image transformation is a broad category of operations that simulate real-world image distortion or deformation.
We leverage the image transformations and verify if the invariance property holds for vision systems.
There are three classes of transformations based on the target space of transformation.

\noindent\textbf{Spatial transformation.} This type of transformation operates on the coordinate space of the input image.
It maps the coordinates of each pixel of the input image to new coordinates within the image by using geometric operation.
A typical spatial transformation is rotation (one type of affine transformation~\cite{annadurai2007fundamentals}) that applies a linear transformation matrix on the coordinates of the input image (see Section~\ref{subsec:affine} for details).

\noindent\textbf{Pixel transformation.} This type of transformation operates on the pixel space of the input image.
It directly changes the pixel values of the input image. 
Each transformed pixel's value depends on only the corresponding input pixel value.
A typical transformation is changing brightness of the input image, where each pixel is added a same amount (see Section~\ref{sec:methodology} for details).

\noindent\textbf{Spatial-pixel transformation.} This type of transformation mix the feature of previous two.
It still operates on the pixel space where it changes the pixel values directly. However, the changes on pixel values also depend on the corresponding coordinates.
A typical example is image smoothing (one type of convolution operation \cf Section~\ref{sec:methodology}) where the output pixel value is the average of the pixel values surround the input pixel.

\begin{comment}
Essentially most transformations can be expressed as composition of two functions T(I, \theta1, \theta2)=[$\forall$ pixels p for each x \in CF(pos(p), \theta1) TF(intensity(p_i,....p_j). the critical

For each pixel p in I
  low, high=CF(coordinate(p, I), theta_1)
  coordinate(low, high)
  low1, high1 = IF(low, high, I, theta_2)  
  Intensity = (low1, high1)
  O[coordinate(p, I)] = IF(low, high, I, theta_2) 
 
Join function all values of theta1 U theta2. Evaluate the output for all of the thetas.

for each critical value of theta what are the allowed values for each pixel. It will be union. 
theta is continuous but the pixel intensity and coordinates are discrete.
For bias: CF is identity function and i=1 IF(N_1) = I[n_1]+theta 

For each operation we need to estimate the possible values IF can take
\end{comment}



==> discussion.tex <==
\section{Discussion}
\label{sec:discuss}

\noindent\textbf{Critical parameter values.}
\sys is based on the explicit model checking that dynamically explores all possible transformed images in the transformation space.
It can produce verified guarantees with no false positive, however with the cost of relatively expensive large space enumeration.
Static analysis with whitebox access~\cite{pei2017deepxplore,szegedy2013intriguing,goodfellow2014explaining,papernot2016limitations,carlini2017towards} to the internals of the system, \eg neural network's trained parameters, can potentially check over an defined input region efficiently with guided search.
The main disadvantage of the static analysis with guided search is that it over-approximates the input region with first-order derivate (gradient) and coarse-grained step size (in gradient descent). This technique trades verified guarantees with efficiency and can thus lead to false positives.
Combining these two methods and leveraging both advantages, \eg efficiency and formal guarantees, is an interesting future direction that we plan to study.

\noindent\textbf{Transformation composition.}
Real-world distortion and deformation often do not come with only single transformation.
Our technique can also support verifying multiple properties with transformations combined together, where the critical parameter values $\mathbb{C}_{critical}$ of transformation composition blow up to the Cartesian crossproduct of each individual $\mathbb{C}_{critical}$.
For example, consider rotate then reflection, where we assume rotation has $|\mathbb{C}_{critical}^{rotation}|=r$, and reflection has $|\mathbb{C}_{critical}^{reflection}|=3$.
In this composition, we have total $|\mathbb{C}_{critical}^{rotation}\times\mathbb{C}_{critical}^{reflection}|=r\times 3$ total pair of critical parameter values to enumerate and verify, which as shown in Section~\ref{sec:reduction}, is still in polynomial with the image size.

In the evaluation, we have shown that composition of multiple transformations may potentially introduce more violations than the simple Cartesian product of violations of each individual transformation.
This indicates we cannot simply compute the Cartesian product of the violations and requires to enumerate the Cartesian product of all critical parameter values of each transformation and check the violations for composition.
Although it is still in polynomial with the image size, it can blow up to very high order of polynomial (\eg shear then rotate has $O(n^5)$).
How to leverage specific properties of multiple transformations to further reduce the composition parameter space to enable efficient model checking is another interesting direction.
In Appendix， we show one possible solution for reducing parameter space of combining reflection and rotation.





==> formal.tex <==
\section{A General Framework for Evaluating ML Robustness}
The goal of any testing or verification technique for ML systems is to measure that ML systems behave correctly under a wide range of corner case scenarios. Note that the incorrect behaviors of ML systems is in essence similar to logic bugs in traditional software. In traditional software, logic bugs are usually detected by testing/verifying the system against specifications user-specified invariants


The goal is to verify a wide variety of user specified invariants (e.g., any image rotation between +90 to -90 should not change the image's class)  

However, writing complete specifications for ML systems is not possible as 


\subsection{Threat Model}

Threat model has two parameters:
  
\begin{itemize}
\item The transformation on input, denoted $t$.  The attacker can
  transform the input using $t$, which can be changing the RGB values of
  some pixels, darkening or lightening of an image, rotating an image,
  adding or removing instructions from a software binary.  $t$ can also be
  some composition of the transformations such as darkening followed by
  rotating.  Here we allow more transformations than previous adversarial
  machine learning work (only changing RGB values of a few pixels).

\item The amount of transformation the attacker is allowed to do, denoted
  $\delta$.  The amount is defined on a distance function, denoted
  $dist_t$.  For adversarial machine learning where a small number of
  pixels are manipulated, the distance can be $L_1$, $L_2$, or
  $L_\infty$ norm.  
For other transformations such as rotation, these distance functions do not make much sense.  We can instead use affine transformation parameterized by the transformation parameters (\eg rotation degrees) and then put distance functions on these transformations parameters (\eg no more than 10 rotation degrees), which we will show later in the paper.

\end{itemize}

\subsection{Robustness Invariant}

Given an input $x$ and a machine learning algorithm  $f$, the output $f(x)$
typically is either a label or a numerical value.  If $f$ outputs a
label, we expand it to output all labelseach with a probability.

A robustness invariant compares $f(x)$ and $f(t(x))$ and determines if
their difference is acceptable.  The invariant can have many forms.  Some
examples are shown below; there can be many more.

\begin{itemize}

\item Suppose the probability for the top label in $f(t(x))$ is $p_{t}$.
      Suppose the probability for the top label in $f(x)$ is $p$.
      Then $p_t >= p$.  That is, transformation should not reduce the probability of top label

\item The label with highest probability in $f(t(x))$ must be the same with that of $f(x)$.

\item The label with highest probability in $f(t(x))$ must be one of the top-$k$ labels in $f(x)$.

\item The numerical values differ less than a small constant: $|f(x) - f(t(x))| < \epsilon $.

\end{itemize}

These invariants are more general than what prior adversarial machine
learning verifies (the first invariant of same label).

\subsection{Taxonomy of ML Robustness}

Given the thread model and the robustness invariants, there are different
levels of robustness a machine learning algorithm can achieve.

{\bf Global robustness.} For all possible input, invariants hold.

{\bf Probabilistic robustness.}  For all possible input, invariants hold
with high probability.

{\bf Local robustness.} For all possible input in a given input set,
invariants hold.

\subsection{Applications of This Framework}

{\bf Verification ML robustness.}  Can take an input set,
(exhaustively) apply the transformation with limit $\delta$, and check
invariants

{\bf Techniques to improve ML robustness.}  For instance, construct neural
network such that an input $x$ and all its variants under the threat model
map to the same label.

{\bf YJF:} Questions: (1) is there probabilistic DNN?  (2) what are the
typical approaches to increase robustness?



